Unitary long-time evolution with quantum renormalization groups and artificial neural networks

In this work we combine quantum renormalization group approaches with deep artificial neural networks for the description of the real-time evolution in strongly disordered quantum matter. We find that this allows us to accurately compute the long-time coherent dynamics of large, many-body localized systems in non-perturbative regimes including the effects of many-body resonances. Concretely, we use this approach to describe the spatiotemporal buildup of many-body localized spin glass order in random Ising chains. We observe a fundamental difference to a non-interacting Anderson insulating Ising chain, where the order only develops over a finite spatial range. We further apply the approach to strongly disordered two-dimensional Ising models highlighting that our method can be used also for the description of the real-time dynamics of nonergodic quantum matter in a general context.

==> quantum_circuit.tex <==
\textit{Time-dependent unitaries.}
To derive the time-dependence of $U^{(k)}(t)$ we express the time-evolution operator in the rotated basis of the first RG-iteration,
\[
e^{-i H t} = e^{-S_1} e^{-i H^{(1)} t} e^{S_1} = e^{-i H^{(1)} t} e^{-S_1(t)} e^{S_1}.
\]
By repeating the above rotation for the factor $e^{-i H^{(k)} t}$ and identifying $U^{(k)}(t) = e^{-S_k(t)} e^{S_k}$ the expression above takes the desired form given in \eqref{eq:psi_t}.
Care has to be taken in evaluating $S_k(t)$ since $H^{(k)}$ is not fully classical.
Nevertheless, it can be approximated semi-analytically by means of the Baker-Campbell-Hausdorff formula, see details in the appendix.

%To derive the time-dependence of $U^{(k)}(t)$ we express the time-evolution operator in the interaction picture of the first RG-iteration,
%\begin{equation}
%e^{-iHt} = e^{-i \bar H t} e^{-i H_0 t}\ \mathcal T e^{-i \int_0^t V(t') dt' },
%\end{equation}
%where $\bar H$ denotes the complementary part of the system, that is unaffected by the first iteration, and $\mathcal T$ is the time-ordered product. 


